A Dataflow Compiler for Efficient LLM Inference using Custom Microscaling Formats

Model quantization represents both parameters (weights) and intermediate values (activations) in a more compact format, thereby directly reducing both computational and memory cost in hardware. The quantization of recent large language models (LLMs) faces challenges to achieve competitive memory density compared to other models such as convolutional neural networks, since values in LLMs require larger dynamic ranges. Current hardware can expedite computation for LLMs using compact numerical formats such as low-bitwidth integers or floating-point numbers. Each has advantages: integer operations simplify circuit design, whereas floating-point calculations can enhance accuracy when a wider dynamic range is required. In this work, we seek an efficient data format that combines the best of both worlds: Microscaling (MX) formats. MX formats are efficient data formats that achieve both large dynamic ranges and high memory density. In this paper, we propose a compiler named MASE for exploring mixed-precision MX formats on dataflow hardware accelerators for LLM inference. Our main contributions are twofold. First, we propose a novel orchestration abstraction to explore both software and hardware optimizations with new data formats. Second, MASE achieves LLM inference at an average precision of 4-bits, with minimal to no accuracy degradation. To our knowledge, MASE represents the first effort to harness fine-grain multi-precision MX formats in the design of LLM hardware accelerators. Over a range of LLMs and datasets, MASE achieves an average improvement of 24% in $\Delta$ accuracy with an overhead of only 3% in energy efficiency compared to designs using 8-bit fixed-point numbers.

==> data/block_size.tex <==



==> data/reb_tables.tex <==





==> imgs/cnn_results.tex <==
\begin{table*}
    \centering
    \caption{Evaluation of MASE on CNN models. We highlight the \best{best} results in each dimension. }
    \label{tab:related_works_cnn}
\resizebox{\textwidth}{!}{%
% \setlength{\tabcolsep}{2pt}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
Model & \multicolumn{3}{c}{ {\tt resnet18} } & \multicolumn{3}{c}{ {\tt resnet50} } & \multicolumn{3}{c}{{\tt mobilenetv2}} & \multicolumn{2}{c}{{\tt mobilenetv3\_small}} & \multicolumn{2}{c}{{\tt mobilenetv3\_large}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
Work & \multicolumn{1}{c}{\cite{sun2022fpga}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{Ours} & \multicolumn{1}{c}{\cite{sun2022fpga}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{Ours} & \multicolumn{1}{c}{\cite{sun2022fpga}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{Ours} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{Ours} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{Ours} \\
Device Class & \multicolumn{1}{c}{FPGA} & \multicolumn{1}{c}{GPU} & \multicolumn{1}{c}{FPGA} & \multicolumn{1}{c}{FPGA} & \multicolumn{1}{c}{GPU} & \multicolumn{1}{c}{FPGA} & \multicolumn{1}{c}{FPGA} & \multicolumn{1}{c}{GPU} & \multicolumn{1}{c}{FPGA}  & \multicolumn{1}{c}{GPU} & \multicolumn{1}{c}{FPGA} & \multicolumn{1}{c}{GPU} & \multicolumn{1}{c}{FPGA} \\
Platform & \multicolumn{1}{c}{ZCU102} & \multicolumn{1}{c}{RTX 3090} & \multicolumn{1}{c}{U250} & \multicolumn{1}{c}{ZCU102} & \multicolumn{1}{c}{RTX 3090} & \multicolumn{1}{c}{U250} & \multicolumn{1}{c}{ZCU102} & \multicolumn{1}{c}{RTX 3090} & \multicolumn{1}{c}{U250}  & \multicolumn{1}{c}{RTX 3090} & \multicolumn{1}{c}{U250} & \multicolumn{1}{c}{RTX 3090} & \multicolumn{1}{c}{U250} \\
\change{Device Count} & \change{ 1 } & \change{ 1 } & \change{ 6 } & \change{ 1 } & \change{ 1 } & \change{ 13 } & \change{ 1 } & \change{ 1 } & \change{ 2 } & \change{ 1 } & \change{ 1 } & \change{ 1 } & \change{ 2 } \\
Quantization & Mixed & float32 & int8 & Mixed & float32 & int8 & Mixed & float32 & int8 & \multicolumn{1}{c}{float32} & \multicolumn{1}{c}{int8} & \multicolumn{1}{c}{float32} & \multicolumn{1}{c}{int8} \\
Accuracy & \best{70.5} & 69.6 & 68.5 & 77.3 & 75.8 & \best{78.1} & 65.7 & \best{72.0} & 70.8 & \best{67.4} & 60.1 & \best{75.2} & 69.9 \\
DSP & 2092 & - & - & 2092 & - & - & 2092 & - & - & - & - & - & - \\
kLUTs & \best{180.1} & - & 6535 & \best{180.1} & - & 11437 & \best{180.1} & - & 1768 & - & 792 & - & 1856 \\
Area Factor & \best{389.3} & - & 6535 & \best{389.3} & - & 11437 & \best{389.3} & - & 1768 & - & 792 & - & 1856\\
Fmax - MHz & 150 & - & \best{250} & 150 & - & \best{250} & 150 & - & \best{250} & - & 280 & - & 240\\
Power (W) & \best{13} & 153 & 427 & \best{13} & 262 & 890 & \best{13} & 211 & 137 & 126 & \best{56} & 204 & \best{131} \\
Frame Rate (FPS) & 215 & \best{4940} & 4725 & 109 & 1665 & \best{4340} & 538 & 4550 & \best{4893} & \best{16308} & 5488 & \best{5958} & 1813 \\
Throughput (GOPS) & 779 & \best{17963} & 17182 & 891 & 13675 & \best{35635} & 320 & 2798 & \best{3009} & \best{1902} & 640 & \best{2651} & 807\\
GOPS/Area Factor & 2.0 & - & \best{2.6} & 2.3 & - & \best{3.1} & 0.8 & - & 1.7  & - & 0.8 & - & 0.4 \\
GOPS/W & 60.4 & \best{117.4} & 40.2 & \best{69.1} & 52.2 & 40.0 & \best{24.8} & 13.3 & 22.0 & \best{15.1} & 11.4 & \best{13.0} & 6.2\\
FPS/W & 16.7 & \best{32.3} & 11.1 & \best{8.5} & 6.4 & 4.9 & \best{41.7} & 21.6 & 35.8 & \best{129.4} & 98.0 & \best{29.2} & 13.8\\
\bottomrule
\end{tabular}
}
\end{table*}

==> imgs/hardware_dse.tex <==
% \begin{figure*}
% \centering
% \begin{minipage}[b]{0.36\textwidth}
% \centering
% \input{imgs/bert_small_dse}
% \caption*{{\footnotesize \tt BERT-BASE}}
% \label{fig:bert_small_dse}
% \end{minipage}
% \begin{minipage}[b]{0.32\textwidth}
% \centering
% \input{imgs/opt125m_dse}
% \caption*{{\footnotesize \tt OPT-125M}}
% \label{fig:opt125m_dse}
% \end{minipage}
% \begin{minipage}[b]{0.3\textwidth}
% \centering
% \input{imgs/llama160m_dse}
% \caption*{{\footnotesize \tt LLaMA-160M}}
% \label{fig:llama160m_dse}
% \end{minipage}
% \caption{Hardware design space for the many-FPGA designs, ranging from a few devices to hundreds of devices. Here we present {\tt BERT}, {\tt OPT} and {\tt LLaMA} for example. Solid dots represent the tested hardware designs and the hollow dots represent the estimated hardware designs due to unavaiable hardware resources. Compared to {\tt Int8}, our quantized models in mixed-precision {\tt MXInt} achieves the same performance with fewer resources.}
% \label{fig:hardware_dse}
% \end{figure*}

==> imgs/large_model_results.tex <==
\begin{table*}
\caption{Comparison with four GPU devices for 7B LLMs. MASE adopts a custom type named MSFP6 (block size of 16, 8-bit exponent, and 6-bit mantissa), which outperforms all other works in energy efficiency. The state-of-the-art {\tt LLM.int8} on GPUs uses {\em tensor core hardware with manually implemented CUDA kernels} for the ``gather" and ``scatter" operations, and performs floating point multiplications, while our FPGA solution by MASE achieves high energy efficiency by automatically deploying new arithmetic types.
}
\label{tab:overall_results}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Models}} & \multicolumn{2}{c}{4 GPUs ({\tt Float32})} & \multicolumn{3}{c}{4 GPUs ({\tt LLM.int8}~\cite{dettmers2022llmint8})} & \multicolumn{3}{c}{$<$30 FPGAs ({\tt int8})} & \multicolumn{3}{c}{$<$30 FPGAs ({\tt MSFP6} \cite{darvish2020pushing})} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-9}
\cmidrule(lr){10-12}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{FPS/W} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{FPS/W} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{FPS/W} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{FPS/W} & \multicolumn{1}{c}{$\times$} \\ \midrule
OPT-2.7B & 0.51 & 0.051 & 0.51 & 0.051 & 1.0 & \best{0.58} & 0.030 & 0.6 & 0.53 & 0.135 & \best{2.6} \\
OPT-6.7B & 0.76 & 0.008 & 0.76 & 0.029 & 3.6 & 0.49 & 0.008 & 1.0 & \best{0.77} & 0.053 & \best{6.6} \\
LLaMA-7B & \best{0.83} & 0.008 & \best{0.83} & 0.036 & 4.5 & 0.53 & 0.008 & 1.0 & 0.79 & 0.039 & \best{4.8} \\
Vicuna-7B & \best{0.84} & 0.008 & \best{0.84} & 0.036 & 4.5 & 0.56 & 0.008 & 1.0 & 0.73 & 0.039 & \best{4.8} \\
Alpaca-7B & \best{0.89} & 0.008 & 0.85 & 0.036 & 4.5 & 0.56 & 0.008 & 1.0 & 0.83 & 0.039 & \best{4.8} \\
\bottomrule
\end{tabular}
% }
\end{table*}



==> imgs/llama_alg.tex <==
\begin{algorithm}[H]
\caption{A transformer block of {\tt Vicuna-7B}.}
{
\footnotesize
\begin{algorithmic}[1]
\Require $X$ \Comment{Input features}
\Require $H$ \Comment{Number of heads}
\State $X_n \gets LayerNorm(X) $
\For{$i \in [0, H)$}
\State $\varied{Q_i} \gets W_{Q_i}X_n$
\State $\varied{K_i} \gets W_{K_i}X_n$ 
\State $\varied{V_i} \gets W_{V_i}X_n$ 
\State $Q'_i \gets RoPE(\varied{Q_i}$)
\State $K'_i \gets RoPE(\varied{K_i}$)
\State $\varied{A_i} \gets \frac{Q'_i{K'_i}^T}{\sqrt{d_k}} $
\State $\hat{A}_i \gets softmax(A_i) $
\State $\varied{B_i} \gets \varied{V_i}\hat{A}_i $
\EndFor
\State $B_c \gets concat(\varied{B_0..B_{H-1}})$
\State $\varied{B_o} \gets W_0B_c$
\State $B_n \gets RMSNorm(\varied{B_o} + X_n) $
\State $\varied{G} \gets W_GB_n$
\State $\varied{U} \gets W_UB_n$
\State $\varied{D} \gets W_D(SiLU(\varied{G} \bigotimes \varied{U}))$
\State $\varied{O} \gets \varied{D} + \varied{B_o} + X$
\State \Return $O$
\end{algorithmic}}
\label{alg:transformer}
\end{algorithm}

==> imgs/mase_dse.tex <==
% \begin{subfigure}[b]{0.32\textwidth}
% \centering
% \input{imgs/dse/resnet50_dse}
% \caption{{\tt resnet50}}
% \label{fig:resnet50_dse}
% \end{subfigure}
% \begin{subfigure}[b]{0.32\textwidth}
% \centering
% \input{imgs/dse/OPT125m_dse}
% \caption{{\tt bert-base-uncased}}
% \label{fig:bert_base_dse}
% \end{subfigure}
% \begin{subfigure}[b]{0.32\textwidth}
\begin{subfigure}[b]{0.45\textwidth}
\centering

\end{subfigure}


==> imgs/model_spec.tex <==
\begin{table*}
    \centering
    \caption{The specifications for the ML models evaluated in this work. float32 = 32-bit floating-point. int8 = 8-bit fixed point. ft = fine-tuned. $^*$The accuracy of models for language modelling was measured in perplexity (smaller is better). \jc{Need to update for ASPLOS}}
    \label{tab:model_specs}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllrrrrrr}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{Category} & \multirow{2}{*}{Task} & \multirow{2}{*}{Name} & \multirow{2}{*}{Sub-style} & \multirow{2}{*}{Dataset} & \multicolumn{1}{l}{\multirow{2}{*}{FLOPs (G)}} & \multicolumn{1}{l}{\multirow{2}{*}{Parameters (M)}} & \multicolumn{4}{c}{Accuracy/perplexity} \\ 
\cmidrule(lr){9-12}
 &  &  &  &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{f32} & \multicolumn{1}{l}{f32 ft} & \multicolumn{1}{l}{int8} & \multicolumn{1}{l}{int8 ft} \\
\midrule
1 & \multirow{6}{*}{CNN} & \multirow{6}{*}{Classification} & \multirow{2}{*}{ResNet} & {\tt resnet18} & \multirow{6}{*}{ImageNet} & 3.64 & 11.7  & 69.6 & -  & 58.6 & 68.5 \\
2 &  &  &  & {\tt resnet50} &  & 8.21 & 25.6 & 75.8 & - & 69.4 & 78.1 \\
3 &  &  & MobileNetV2 &{\tt mobilenetv2} &  & 0.615 & 3.50 & 72.0 & - & 58.8 & 70.8 \\
4 &  &  & \multirow{2}{*}{MobileNetV3} & {\tt mobilenetv3\_small} & & 0.117 & 2.54 & 67.4 & - & - & 60.1  \\
5 &  &  &  & {\tt mobilenetv3\_large} &  & 0.445 & 5.48 & 75.2 & -  & - & 69.9 \\
% 6 &  &  & EfficientNet & {\tt efficientnet\_v2\_s} &  & 10.7 & 21.5 & 83.9 & - & - & 71.8 \\
\midrule
6 & \multirow{5}{*}{Transformers} & \multirow{2}{*}{Question Answering} & \multirow{2}{*}{BERT} & {\tt bert-base-cased} & \multirow{2}{*}{QNLI} & 22.4 & 108 & 90.5 & -  & 49.5 & 75.3 \\
7 &  &  &  &  {\tt bert-large-cased} &  & 79.0 & 334 & 92.7 & - & 51.3 & 56.0 \\
\cmidrule(lr){3-12}
8 &  &  \multirow{3}{*}{Language Modelling} & \multirow{3}{*}{OPT} & {\tt facebook/opt-125m} & \multirow{3}{*}{WikiText2} & 32.3 & 125 & 60.3$^*$ & 21.4$^*$ & 553$^*$ & 27.9$^*$ \\
9 &  &  &  & {\tt facebook/opt-350m} &  & 85.8 & 331 & 48.7$^*$ & 18.3$^*$ & 7.42k$^*$ & 26.0$^*$ \\
10 &  &  &  & {\tt facebook/opt-1.3b} &  & 339 & 1316 & 32.1$^*$ & - & 8.28k$^*$ & - \\
\bottomrule
\end{tabular}
}
\end{table*}

==> imgs/model_specs.tex <==
\begin{table*}
    \centering
    \caption{The specifications for the ML models evaluated in this work. float32 = 32-bit floating-point. int8 = 8-bit fixed point. ft = fine-tuned. $^*$The accuracy of models for language modelling was measured in perplexity (smaller is better). }
    \label{tab:model_specs}
\resizebox{\textwidth}{!}{%
% \setlength{\tabcolsep}{2pt}
%     \begin{tabular}{lllrrrrrrrrrr}
% \toprule
% \multirow{2}{*}{} & \multirow{2}{*}{Categories} & \multirow{2}{*}{Models} & \multicolumn{4}{c}{Accuracy} & \multicolumn{6}{c}{Hardware Results} \\
% \cmidrule(lr){4-7}
% \cmidrule(lr){8-13}
%  &  &  & \multicolumn{1}{c}{float32} & \multicolumn{1}{c}{int8} & \multicolumn{1}{c}{float32(ft)} & \multicolumn{1}{c}{int8(ft)} & \multicolumn{1}{c}{Devices} & \multicolumn{1}{c}{LUTs} & \multicolumn{1}{c}{Registers} & \multicolumn{1}{c}{Cycles} & \multicolumn{1}{c}{Fmax} & \multicolumn{1}{c}{Throughput} \\
%  \midrule
% 1 & \multirow{6}{*}{CNN} & {\tt resnet18} &  &  &  &  &  &  &  &  &  & \\
% 2 &  & {\tt resnet50         } &  &  &  &  &  &  &  &  &  & \\
% 3 &  & {\tt mobilenetv2      } &  &  &  &  &  &  &  &  &  & \\
% 4 &  & {\tt mobilenetv3\_small} &  &  &  &  &  &  &  &  &  & \\
% 5 &  & {\tt mobilenetv3\_large} &  &  &  &  &  &  &  &  &  & \\
% 6 &  & {\tt efficientnet\_v2\_s} &  &  &  &  &  &  &  &  &  & \\
% \midrule
% %7 &  & {\tt efficientnet\_v2\_m} &  &  &  &  &  &  &  &  &  & \\
% %8 &  & {\tt efficientnet\_v2\_l} &  &  &  &  &  &  &  &  &  & \\
% 7 & \multirow{5}{*}{Transformers} & {\tt bert-base-uncased} &  &  &  &  &  &  &  &  &  & \\
% 8 &  & {\tt bert-large-uncased}&  &  &  &  &  &  &  &  &  & \\
% 9 &  & {\tt facebook/opt-125m }&  &  &  &  &  &  &  &  &  & \\
% 10 &  & {\tt facebook/opt-350m }&  &  &  &  &  &  &  &  &  & \\
% 11 &  & {\tt facebook/opt-1.3b }&  &  &  &  &  &  &  &  & & \\
% \bottomrule
% \end{tabular}
\begin{tabular}{llllllrrrrrr}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{Category} & \multirow{2}{*}{Task} & \multirow{2}{*}{Name} & \multirow{2}{*}{Sub-style} & \multirow{2}{*}{Dataset} & \multicolumn{1}{l}{\multirow{2}{*}{FLOPs (G)}} & \multicolumn{1}{l}{\multirow{2}{*}{Parameters (M)}} & \multicolumn{4}{c}{Accuracy/perplexity} \\ 
\cmidrule(lr){9-12}
 &  &  &  &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{f32} & \multicolumn{1}{l}{f32 ft} & \multicolumn{1}{l}{int8} & \multicolumn{1}{l}{int8 ft} \\
\midrule
1 & \multirow{6}{*}{CNN} & \multirow{6}{*}{Classification} & \multirow{2}{*}{ResNet} & {\tt resnet18} & \multirow{6}{*}{ImageNet} & 3.64 & 11.7  & 69.6 & -  & 58.6 & 68.5 \\
2 &  &  &  & {\tt resnet50} &  & 8.21 & 25.6 & 75.8 & - & 69.4 & 78.1 \\
3 &  &  & MobileNetV2 &{\tt mobilenetv2} &  & 0.615 & 3.50 & 72.0 & - & 58.8 & 70.8 \\
4 &  &  & \multirow{2}{*}{MobileNetV3} & {\tt mobilenetv3\_small} & & 0.117 & 2.54 & 67.4 & - & - & 60.1  \\
5 &  &  &  & {\tt mobilenetv3\_large} &  & 0.445 & 5.48 & 75.2 & -  & - & 69.9 \\
% 6 &  &  & EfficientNet & {\tt efficientnet\_v2\_s} &  & 10.7 & 21.5 & 83.9 & - & - & 71.8 \\
\midrule
6 & \multirow{5}{*}{Transformers} & \multirow{2}{*}{Question Answering} & \multirow{2}{*}{BERT} & {\tt bert-base-cased} & \multirow{2}{*}{QNLI} & 22.4 & 108 & 90.5 & -  & 49.5 & 75.3 \\
7 &  &  &  &  {\tt bert-large-cased} &  & 79.0 & 334 & 92.7 & - & 51.3 & 56.0 \\
\cmidrule(lr){3-12}
8 &  &  \multirow{3}{*}{Language Modelling} & \multirow{3}{*}{OPT} & {\tt facebook/opt-125m} & \multirow{3}{*}{WikiText2} & 32.3 & 125 & 60.3$^*$ & 21.4$^*$ & 553$^*$ & 27.9$^*$ \\
9 &  &  &  & {\tt facebook/opt-350m} &  & 85.8 & 331 & 48.7$^*$ & 18.3$^*$ & 7.42k$^*$ & 26.0$^*$ \\
10 &  &  &  & {\tt facebook/opt-1.3b} &  & 339 & 1316 & 32.1$^*$ & - & 8.28k$^*$ & - \\
\bottomrule
\end{tabular}
}
\end{table*}

==> imgs/motivation_table.tex <==
\begin{figure}
\centering
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{imgs/first_page.pdf}  
    \caption{\footnotesize Examples of MiniFloat and Microscaling formats.}
    \label{fig:arithmatic_examples}
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
\centering
% \resizebox{0.45\textwidth}{!}{%
\vspace{1em}
% \resizebox{\textwidth}{!}{%
{\footnotesize
\begin{tabular}{ccrrr}
\toprule
Approaches & Config & \multicolumn{1}{c}{Perplexity} & \makecell[c]{Memory \\ Density} & \makecell[c]{Arithmetic \\ Density} \\
\midrule
{\tt Float32} & - & \best{7.06} & 1$\times$ & 1$\times$ \\
\midrule
\tt{Int8} & W8A8 & 265 & 4$\times$ & 7.7$\times$ \\
{\tt LLM.int8()} & W8A8$^*$ & \best{7.06} & 2$\times$ & 1.24$\times$ \\
{\tt LLM.int4()} & W4A4$^*$ & 7.43 & 2$\times$ & 1.46$\times$ \\
\midrule
\tt{MF8} & W8A8 & 7.18 & 4$\times$ & 17.4$\times$ \\
% Denormalized MF & W8A8 & 7.37 & 4$\times$ & 17.4$\times$ \\
\tt{MXInt8} & W8A8 & \best{7.07} & 3.8$\times$ & 14.4$\times$ \\
\tt{BMF8} & W8A8 & 223k & 3.8$\times$ & 14.4$\times$ \\
\tt{BL8} & W8A8 & 18.8 & 3.8$\times$ & 16.1$\times$ \\
\bottomrule
\end{tabular}
}
\caption{\footnotesize
Evaluation of these formats in similar average bits for quantizing {\tt LLaMA-7B} on {\tt Wikitext2}. Small perplexity means better LLM performance. Higher memory density or hardware arithmetic density means better hardware efficiency~\cite{darvish2020pushing}. $^*$ means the inliner matrix multiplications are calculated in fixed-point, and outliers are calculated in {\tt Float16}.}
\label{tab:arithmatic_examples}
\end{subfigure}
\caption{Comparison between MiniFloat and Microscaling formats. We observe that MXInt has shown significant advantages in {\em both minimizing accuracy loss and maximizing hardware efficiency.} Our work exploits mixed-precision MXInt formats in reconfigurable hardware accelerators for LLM inference.}
\label{fig:first_page}
\end{figure}

==> imgs/overall_result_table.tex <==
\begin{table*}[]
\caption{Comparison between the quantized model into mixed-precision {\tt MXInt} on many-FPGA systems (connected using QSFP28) and the vanilla model in {\tt LLM.int8()}~\cite{dettmers2022llm} on multi-GPU systems (connected using PCIE). 
% The upper part of the table runs the whole model on a many-FPGA system. The lower part of the table runs a few blocks of the model on the many-FPGA system due to limited FPGA resources, and iterates computation for running the whole model. 
Our approach shows significant improvement in both throughput and energy efficiency compared to GPUs. TPS = token per second. TPS/W = token per Joule.}
\label{tab:overall_results}
\centering
\resizebox{\textwidth}{!}{%
% {\footnotesize
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Models}} & \multicolumn{7}{c}{Our Work} & \multicolumn{3}{c}{GPU} & \multicolumn{2}{c}{Normalized to GPU} \\
\cmidrule(lr){2-8}
\cmidrule(lr){9-11}
\cmidrule(lr){12-13}
& \multicolumn{1}{c}{Devices} & \multicolumn{1}{c}{LUTs} & \multicolumn{1}{c}{DSPs} & \multicolumn{1}{c}{BRAM} & \multicolumn{1}{c}{URAM} & \multicolumn{1}{c}{TPS} & \multicolumn{1}{c}{TPS/W} & \multicolumn{1}{c}{Devices} & \multicolumn{1}{c}{TPS} & \multicolumn{1}{c}{TPS/W} & \multicolumn{1}{c}{TPS} & \multicolumn{1}{c}{TPS/W} \\
\midrule
{\tt LLaMA-160M} & 30 & 43.6M & 75.5k & 7.4k & 1.8k & \best{781k} & \best{339.20} & 4 & 315k & 227.37 & 2.27$\times$ & 1.49$\times$ \\
{\tt BERT-BASE } & 25 & 34.8M & 49.4k & 5.2k & 1.3k & \best{781k} & \best{414.98} & 4 & 298k & 214.16 & 2.62$\times$ & 1.94$\times$ \\
{\tt BERT-LARGE} & 16 & 24.8M & 34.0k & 15.8k & 3.9k & \best{146k} & \best{114.56} & 4 & 116k & 83.20 & 1.26$\times$ & 1.38$\times$\\
{\tt OPT-125M  } & 26 & 38.9M & 57.2k & 6.0k & 1.5k & \best{586k} & \best{293.76} & 4 & 303k & 218.88 & 1.93$\times$ & 1.34$\times$ \\
{\tt OPT-350M  } & 19 & 28.4M & 38.7k & 15.3k & 3.7k & \best{145k} & \best{97.41} & 4 & 118k & 86.08 & 1.23$\times$ & 1.13$\times$ \\
{\tt OPT-1.3B  } & 19 & 29.1M & 27.3k & 73.7k & 17.7k & 36.6k & 21.59 & 4 & \best{54.7k} & \best{39.68} & 0.67$\times$ & 0.54$\times$ \\
{\tt OPT-2.7B }& 27 & 41.7M & 46.7k & 65.3k & 15.7k & \best{29.3k} & \best{9.72} & 4 & 4.35k & 6.14 & 6.74$\times$ & 1.58$\times$ \\
\midrule
{\bf Geom. Mean} & 22 & 33.3M & 46.5k & 17.0k & 5.3k & \best{290k} & \best{164.58} & 4 & 133k & 98.65 & 2.04$\times$ & 1.29$\times$ \\
\midrule
{\tt OPT-6.7B }& 29 & 39.1M & 50.9k & 40.3k & 9.9k & \best{9.37k} & \best{6.16} & 4 & 2.82k & 3.71 & 3.32$\times$ & 1.66$\times$\\
{\tt LLaMA-7B }& 28 & 36.3M  & 75.3k & 41.6k & 10.0k & \best{9.15k} & \best{5.64} & 4 & 3.58k & 4.61 & 2.56$\times$ & 1.23$\times$ \\
{\tt Vicuna-7B} & 29 & 37.7M & 70.8k & 40.4k & 9.8k & \best{9.15k} & \best{5.45} & 4 & 3.71k & 4.61 & 2.47$\times$ & 1.18$\times$\\
{\tt Alpaca-7B} & 29 & 37.9M & 70.7k & 41.6k & 10.0k & \best{9.15k} & \best{5.44} & 4 & 3.71k & 4.61 & 2.47$\times$ & 1.18$\times$\\
\midrule
{\bf Geom. Mean} & 29 & 37.8M & 66.4k & 41.0k & 9.9k & \best{9.20k} & \best{5.67} & 4 & 3.43k & 4.37 & 2.73$\times$ & 1.33$\times$ \\
\bottomrule
\end{tabular}}
\end{table*}

==> imgs/reb_tables.tex <==





==> imgs/self_compare.tex <==
\begin{table}[t]
\centering
\caption{A comparison between mixed-precision {\tt MXInt} with other approaches in accuracy and average bitwidth on {\tt SST2} task. 
% The upper part of the table runs the whole model on a many-FPGA system. The lower part of the table runs a few blocks of the model on the many-FPGA system due to limited FPGA resources, and iterates computation for running the whole model. 
$^*$ means the models are fine-tuned and quantized before evaluation, and $^\dag$ denotes the models are quantized and evaluated in zero-shot prompting style.  We highlight the \best{best} results after quantization. {\tt FP32} = {\tt Float32}.}
\label{tab:self_compare}
\resizebox{0.48\textwidth}{!}{%
% {\footnotesize
\begin{tabular}{lrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Models}} & \multicolumn{4}{c}{Accuracy} & \multicolumn{2}{c}{Average Bitwidth} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-7}
& \multicolumn{1}{c}{{\tt Int8}} & \makecell[c]{ Mixed \\ {\tt Int}} & \makecell[c]{ Mixed \\ {\tt MXInt}} & \multicolumn{1}{c}{ {\tt FP32}} & \makecell[c]{ Mixed \\ {\tt Int}} & \makecell[c]{ Mixed \\ {\tt MXInt}} \\
\midrule
{\tt LLaMA-160M}$^*$ & 0.8 & 0.72     & \best{0.87} & 0.91 & 7 & \best{4.8} \\
{\tt BERT-BASE}$^*$ & 0.9 & 0.74      & \best{0.91} & 0.93 & 7.6 & \best{4.4} \\
{\tt BERT-LARGE}$^*$ & 0.74 & 0.65    & \best{0.89} & 0.92 & 7.5 & \best{4.3}  \\
{\tt OPT-125M}$^*$ & 0.91 & 0.63      & \best{0.88} & 0.92 & 6.8  & \best{4.4} \\
{\tt OPT-350M}$^*$  & 0.94 & 0.89     & \best{0.91} & 0.94 & 6.5 & \best{4.4} \\
{\tt OPT-1.3B}$^{\dag}$ & 0.52 & 0.60 & \best{0.76} & 0.82 & 6.7 & \best{5.1} \\
{\tt OPT-2.7B}$^\dag$ & 0.58 & 0.54  & \best{0.63} & 0.51 & 8.9 & \best{4.4}  \\
\midrule
\textbf{Geom. Mean.} & 0.74 & 0.67 & \best{0.83} & 0.86 & 7.18 & \best{4.77} \\
\midrule
{\tt OPT-6.7B}$^\dag$ & 0.49 & 0.54 & \best{0.73} & 0.76 & 4.7 & \best{4.4} \\
{\tt LLaMA-7B}$^\dag$ & 0.53 & 0.63 & \best{0.84} & 0.83 & 4.7 & \best{4.5} \\
{\tt Vicuna-7B}$^\dag$ & 0.53 & 0.59 & \best{0.83} & 0.84 & 5.1  & \best{4.4} \\
{\tt Alpaca-7B}$^\dag$ & 0.56 & 0.59 & \best{0.89} & 0.85 & 5.1 & \best{4.5} \\
\midrule
\textbf{Geom. Mean.} & 0.53 & 0.59 & \best{0.82}& 0.82 & 4.95 & \best{4.45} \\
\bottomrule
\end{tabular}
}
\end{table}


==> imgs/transformer_results.tex <==
\begin{table*}
    \centering
    \caption{Evaluation of MASE on large language models. $\times$ = energy efficiency improvement compared to Float32. We highlight the \best{best} results in comparison. TPS = tokens per second. TPS/W = tokens per Joule.}
    \label{tab:overall_results}
\resizebox{\textwidth}{!}{%

\begin{tabular}{lrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Models}} & \multicolumn{3}{c}{PyTorch (Float32) on 4 GPUs} & \multicolumn{4}{c}{{\tt LLM.int8()}~\cite{dettmers2022llm} on 4 GPUs} & \multicolumn{5}{c}{MASE (MSFP4)} & \multicolumn{5}{c}{MASE (MSFP6)} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-8}
\cmidrule(lr){9-13}
\cmidrule(lr){14-18}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{TPS} & \multicolumn{1}{c}{TPS/W} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{TPS} & \multicolumn{1}{c}{TPS/W} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{\#device} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{TPS} & \multicolumn{1}{c}{TPS/W} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{\#device} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{TPS} & \multicolumn{1}{c}{TPS/W} & \multicolumn{1}{c}{$\times$} \\
\midrule
{\tt BERT-BASE } & \best{0.93} & 211k & 155.68 & 0.02 & 298k & 214.16 & 1.38 & 25 & 0.91 & \best{781k} & \best{407.04} & \best{2.63} & 25 & 0.92 & 587k & 313.60 & 2.02 \\
{\tt BERT-LARGE} & \best{0.92} & 65.2k & 47.36 & \best{0.92} & 116k & 83.20 & 1.76 & 31 & \best{0.92} & \best{294k} & \best{117.76} & \best{2.49} &  19 & \best{0.92} & 146k & 96.00 & 2.03 \\
{\tt OPT-125M  } & \best{0.92} & 218k & 160.00 & 0.02 & 303k & 218.88 & 1.37 & 25 & 0.91 & \best{781k} & \best{414.72} & \best{2.59} & 25 & \best{0.92} & 587k & 313.60 & 1.96 \\
{\tt OPT-350M  } & \best{0.94} & 66.1k & 48.64 & 0.93 & 118k & 86.08 & 1.76 & 31 & 0.93 & \best{294k} & \best{115.20} & \best{2.37} & 19 & 0.93 & 146k & 94.72 & 1.95 \\
{\tt OPT-1.3B  } & \best{0.82} & 18.6k & 14.08 & 0.81 & \best{54.7k} & \best{39.68} & \best{2.81} & 17 & 0.60 & 36.6k & 26.88 & 1.91 & 20 & 0.80 & 36.6k & 23.04 & 1.63 \\
\midrule
{\tt OPT-2.7B  } & 0.51 & 8.83k & 6.53 & 0.51 & 4.35k & 6.14 & 0.94 & 23 & \best{0.53} & \best{23.4k} & \best{12.54} & \best{1.92} & 28 & \best{0.53} & \best{23.4k} & 10.62 & 1.63 \\
{\tt OPT-6.7B  } & 0.76 & 768 & 1.02 & 0.76 & 2.82k & 3.71 & 3.63 & 22 & 0.59 & \best{9.22k} & \best{5.38} & \best{5.25} & 26 & \best{0.77} & \best{9.22k} & 4.61 & 4.50 \\
{\tt LLaMA-7B  } & \best{0.83} & 896 & 1.02 & \best{0.83} & 3.58k & 4.61 & 4.52 & 22 & 0.69 & \best{9.22k} & \best{5.38} & \best{5.25} & 26 & 0.79 & \best{9.22k} & 4.48  & 4.38 \\
{\tt Vicuna-7B } & \best{0.84} & 896 & 1.02 & \best{0.84} & 3.71k & 4.61 & 4.52 & 22 & 0.63 & \best{9.22k} & \best{5.38} & \best{5.25} & 26 & 0.77 & \best{9.22k} & 4.48  & 4.38 \\
{\tt Alpaca-7B } & \best{0.89} & 896 & 1.02 & 0.85 & 3.71k & 4.61 & 4.52 & 22 & 0.78 & \best{9.22k} & \best{5.38} & \best{5.25} & 26 & 0.83 & \best{9.22k} & 4.48  & 4.38 \\
\bottomrule
\end{tabular}
}
\end{table*}
